Time and Space Measures for a Complete Graph Computation Model

We present a computation model based on a subclass of GP 2 graph programs which can simulate any off-line Turing machine of space complexity O(s(n) log s(n)) in space O(s(n)). The simulation only requires a quadratic time overhead. Our model shares this property with Sch\"onhage's storage modification machines and Kolmogorov-Uspenskii machines. These machines use low-level pointer instructions whereas our GP 2-based model uses pattern-based transformation rules and high-level control constructs.

==> eptcsdata.tex <==
\providecommand{\firstpage}{23}
\providecommand{\publicationstatus}{R. Heckel and C.M. Poskitt (Eds.): 13th International\\ Workshop on Graph Computation Models (GCM 2022)\\
EPTCS 374, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.374.4}{10.4204/EPTCS.374.4}}
\pdfoutput=1

